The Perfect Victim: Computational Analysis of Judicial Attitudes towards Victims of Sexual Violence

We develop computational models to analyze court statements in order to assess judicial attitudes toward victims of sexual violence in the Israeli court system. The study examines the resonance of "rape myths" in the criminal justice system's response to sex crimes, in particular in judicial assessment of victim's credibility. We begin by formulating an ontology for evaluating judicial attitudes toward victim's credibility, with eight ordinal labels and binary categorizations. Second, we curate a manually annotated dataset for judicial assessments of victim's credibility in the Hebrew language, as well as a model that can extract credibility labels from court cases. The dataset consists of 855 verdict decision documents in sexual assault cases from 1990-2021, annotated with the help of legal experts and trained law students. The model uses a combined approach of syntactic and latent structures to find sentences that convey the judge's attitude towards the victim and classify them according to the credibility label set. Our ontology, data, and models will be made available upon request, in the hope they spur future progress in this judicial important task.

==> tables/categories.tex <==

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[normalem]{ulem}
% % \useunder{\uline}{\ul}{}
% \begin{table*}[]
% \begin{tabular}{|c|c|c|}
% \hline
% \textbf{}                              & \textbf{High Level}                                                                          & \textbf{Granular Level}                                                           \\ \hline
% Not relevant (27.4\%)                  & Not relevant (27.4\%)                                                                        & Not relevant (27.4\%)                                                             \\ \hline
% \multirow{6}{*}{Credibility (59.6\%)}  & \multirow{2}{*}{Unequivocal credibilitys (36.1\%)}                                           & Unequivocal credibility - no fake allegations, not vengeful (9.0\%)               \\ \cline{3-3} 
%                                        &                                                                                              & Unequivocal credibility - clear, simple, without exaggeration, authentic (27.1\%) \\ \cline{2-3} 
%                                        & \multirow{2}{*}{Credible because - something is strengthening victim's credibility (17.4\%)} & Credible because of external support (8.4\%)                                      \\ \cline{3-3} 
%                                        &                                                                                              & Credible because the accused is less credible (9.0\%)                             \\ \cline{2-3} 
%                                        & \multirow{2}{*}{Credible but - something is undermining victim's credibility (6.1\%)}        & Credible but has some problems (4.8\%)                                            \\ \cline{3-3} 
%                                        &                                                                                              & Credible but cannot convict, sole testimony, no support (1.3\%)                   \\ \hline
% \multirow{2}{*}{Not credible (12.9\%)} & \multirow{2}{*}{Not credible (12.9\%)}                                                       & Not credible because several versions, non consistent (9.0\%)                     \\ \cline{3-3} 
%                                        &                                                                                              & Not credible because vengeful, not authentic, fake (3.9\%)                        \\ \hline
% \end{tabular}
% \caption{Hierarchical structure of the labels in the sentence classification task. The table shows the distribution of the labels at each level, providing insights into the relationships between the different labels.}
% \label{table:train_label_distribution}
% \end{table*}

==> tables/labels.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

